Cofibrations in Homotopy Theory

We define Anderson-Brown-Cisinski (ABC) cofibration categories, and construct homotopy colimits of diagrams of objects in ABC cofibration categories. Homotopy colimits for Quillen model categories are obtained as a particular case. We attach to each ABC cofibration category a left Heller derivator. A dual theory is developed for homotopy limits in ABC fibration categories and for right Heller derivators. These constructions provide a natural framework for 'doing homotopy theory' in ABC (co)fibration categories.

==> cofib-cat-crossref.tex <==
\newcommand{\CrossrefCofibcatchapIntroduction}{vii}
\newcommand{\CrossrefCofibcatsubseccompareabcquillen}{ix}
\newcommand{\CrossrefCofibcatsubsecoutline}{ix}
\newcommand{\CrossrefCofibcatchapCofibrationAndFibrationCategories}{1}
\newcommand{\CrossrefCofibcatsecCofibrationCategoriesFibrationCategoriesAxioms}{1.1}
\newcommand{\CrossrefCofibcatdefncofcat}{1.1.1}
\newcommand{\CrossrefCofibcatdefnfibcat}{1.1.2}
\newcommand{\CrossrefCofibcatdefnabcmodel}{1.1.3}
\newcommand{\CrossrefCofibcatsecsumsproducts}{1.2}
\newcommand{\CrossrefCofibcatlemcofsums}{1.2.1}
\newcommand{\CrossrefCofibcatsecfactlemmas}{1.3}
\newcommand{\CrossrefCofibcatlembrownfact}{1.3.1}
\newcommand{\CrossrefCofibcatrembrownfact}{1.3.2}
\newcommand{\CrossrefCofibcatlemrelativefactorization}{1.3.3}
\newcommand{\CrossrefCofibcatlemrelbrownfact}{1.3.4}
\newcommand{\CrossrefCofibcatsecextlemmas}{1.4}
\newcommand{\CrossrefCofibcatlemgluinglemmaXXY}{1.4.1}
\newcommand{\CrossrefCofibcateqngluinglemmasimplifying}{1.1}
\newcommand{\CrossrefCofibcatlemexcision}{1.4.2}
\newcommand{\CrossrefCofibcatlemequivaxiomcfXXXXY}{1.4.3}
\newcommand{\CrossrefCofibcatseccylobj}{1.5}
\newcommand{\CrossrefCofibcatdefncylobj}{1.5.1}
\newcommand{\CrossrefCofibcatlemexistencecyl}{1.5.2}
\newcommand{\CrossrefCofibcatlemexistencerelcyl}{1.5.3}
\newcommand{\CrossrefCofibcatsectransfincomp}{1.6}
\newcommand{\CrossrefCofibcatdefntranscomp}{1.6.1}
\newcommand{\CrossrefCofibcatlemtransfinitecompositionstability}{1.6.2}
\newcommand{\CrossrefCofibcatlemsmallcofsums}{1.6.3}
\newcommand{\CrossrefCofibcatlemequivformaxiomcfXXXXXXY}{1.6.4}
\newcommand{\CrossrefCofibcatlemtranscompequiv}{1.6.5}
\newcommand{\CrossrefCofibcatlemequivformaxiomcfXXXXXXXY}{1.6.6}
\newcommand{\CrossrefCofibcatseccatoverunder}{1.7}
\newcommand{\CrossrefCofibcatpropovercofcat}{1.7.1}
\newcommand{\CrossrefCofibcatsecproperness}{1.8}
\newcommand{\CrossrefCofibcatdefnpropercofcat}{1.8.1}
\newcommand{\CrossrefCofibcatdefncatweakequiv}{1.8.2}
\newcommand{\CrossrefCofibcatdefnpropercofibration}{1.8.3}
\newcommand{\CrossrefCofibcatthmleftproperstruct}{1.8.4}
\newcommand{\CrossrefCofibcatproppropermapsXXY}{1.8.5}
\newcommand{\CrossrefCofibcatproppropermapsXXXY}{1.8.6}
\newcommand{\CrossrefCofibcatdefnmapretract}{1.8.7}
\newcommand{\CrossrefCofibcatproppropermapsXXXXY}{1.8.8}
\newcommand{\CrossrefCofibcatchapmodcatcatcofobj}{2}
\newcommand{\CrossrefCofibcatdefncatcofobj}{2.1.1}
\newcommand{\CrossrefCofibcatproprelcatcofobj}{2.1.2}
\newcommand{\CrossrefCofibcatdefnllp}{2.2.1}
\newcommand{\CrossrefCofibcatdefnmodelcat}{2.2.2}
\newcommand{\CrossrefCofibcatpropllpcharact}{2.2.3}
\newcommand{\CrossrefCofibcatproprelclosedmodcat}{2.2.4}
\newcommand{\CrossrefCofibcatproprelproperclosedmodcat}{2.2.5}
\newcommand{\CrossrefCofibcatdefnbauescofcat}{2.3.1}
\newcommand{\CrossrefCofibcatproprelcatcofcatbaues}{2.3.2}
\newcommand{\CrossrefCofibcatdefnwaldcofcat}{2.4.1}
\newcommand{\CrossrefCofibcatproprelcatcofcatwaldhausen}{2.4.2}
\newcommand{\CrossrefCofibcatchapexamples}{3}
\newcommand{\CrossrefCofibcatsecexampletopspaces}{3.1}
\newcommand{\CrossrefCofibcateqnexp}{3.1}
\newcommand{\CrossrefCofibcatdefnhomotopy}{3.1.1}
\newcommand{\CrossrefCofibcatdefnhomotopyundera}{3.1.2}
\newcommand{\CrossrefCofibcatdefnhomotopyovera}{3.1.3}
\newcommand{\CrossrefCofibcatdefnhomotequiv}{3.1.4}
\newcommand{\CrossrefCofibcatdefnhep}{3.1.5}
\newcommand{\CrossrefCofibcatlemhurcomp}{3.1.6}
\newcommand{\CrossrefCofibcateqnhep}{3.2}
\newcommand{\CrossrefCofibcateqnhlp}{3.3}
\newcommand{\CrossrefCofibcatlemhurewiczreplace}{3.1.7}
\newcommand{\CrossrefCofibcatlemdold}{3.1.8}
\newcommand{\CrossrefCofibcatlemtrivhurcof}{3.1.9}
\newcommand{\CrossrefCofibcatlemhurpush}{3.1.10}
\newcommand{\CrossrefCofibcatlemhurcolim}{3.1.11}
\newcommand{\CrossrefCofibcatthmhurtop}{3.1.12}
\newcommand{\CrossrefCofibcatthmstromtop}{3.1.13}
\newcommand{\CrossrefCofibcatdefnserrefib}{3.1.14}
\newcommand{\CrossrefCofibcatthmquillentop}{3.1.15}
\newcommand{\CrossrefCofibcatsecexampleabcat}{3.2}
\newcommand{\CrossrefCofibcatlempushabelianXXY}{3.2.1}
\newcommand{\CrossrefCofibcatlempushabelianXXXY}{3.2.2}
\newcommand{\CrossrefCofibcatlemsnake}{3.2.3}
\newcommand{\CrossrefCofibcatthmabcatisabccatXXY}{3.2.4}
\newcommand{\CrossrefCofibcatthmabcatisabccatXXXY}{3.2.5}
\newcommand{\CrossrefCofibcatlemadjabelian}{3.2.6}
\newcommand{\CrossrefCofibcateqnadjabelianXXY}{3.4}
\newcommand{\CrossrefCofibcateqnadjabelianXXXY}{3.5}
\newcommand{\CrossrefCofibcatthmabcatisabccatXXXXY}{3.2.7}
\newcommand{\CrossrefCofibcatthmabcatisabccatXXXXXY}{3.2.8}
\newcommand{\CrossrefCofibcatchapkanextensions}{4}
\newcommand{\CrossrefCofibcatsecfunctorsnaturammaps}{4.1}
\newcommand{\CrossrefCofibcateqncompXXY}{4.1}
\newcommand{\CrossrefCofibcateqncompXXXY}{4.2}
\newcommand{\CrossrefCofibcateqncompXXXXY}{4.3}
\newcommand{\CrossrefCofibcateqncompXXXXXY}{4.4}
\newcommand{\CrossrefCofibcateqncompXXXXXXY}{4.5}
\newcommand{\CrossrefCofibcateqncompXXXXXXXY}{4.6}
\newcommand{\CrossrefCofibcateqncompXXXXXXXXY}{4.7}
\newcommand{\CrossrefCofibcatsecadjointfunctors}{4.2}
\newcommand{\CrossrefCofibcatpropadjfunctors}{4.2.1}
\newcommand{\CrossrefCofibcatpropadjfunctorsXXXY}{4.2.2}
\newcommand{\CrossrefCofibcatsecleftrightkanextension}{4.3}
\newcommand{\CrossrefCofibcatdefndefkanext}{4.3.1}
\newcommand{\CrossrefCofibcatpropexistencekanextension}{4.3.2}
\newcommand{\CrossrefCofibcateqnexistencekanextensionXXY}{4.8}
\newcommand{\CrossrefCofibcateqnexistencekanextensionXXXY}{4.9}
\newcommand{\CrossrefCofibcatpropbasecompositionkanextension}{4.3.3}
\newcommand{\CrossrefCofibcatcorneededbygenhomlim}{4.3.4}
\newcommand{\CrossrefCofibcatchapcatweq}{5}
\newcommand{\CrossrefCofibcatsecwhomotopycat}{5.2}
\newcommand{\CrossrefCofibcatdefnhcat}{5.2.1}
\newcommand{\CrossrefCofibcatdefnhcatXXXY}{2}
\newcommand{\CrossrefCofibcatthmgz}{5.2.2}
\newcommand{\CrossrefCofibcatsecgeneralhomotopicmaps}{5.3}
\newcommand{\CrossrefCofibcatdefnhomotopicmaps}{5.3.1}
\newcommand{\CrossrefCofibcatsecapproximationfunctors}{5.4}
\newcommand{\CrossrefCofibcatdefnwleftapproximation}{5.4.1}
\newcommand{\CrossrefCofibcatlemsufficientcondequiv}{5.4.2}
\newcommand{\CrossrefCofibcatdefnwleftcleavage}{5.4.3}
\newcommand{\CrossrefCofibcatdefnwrightcleavage}{5.4.4}
\newcommand{\CrossrefCofibcatlemcleavagemap}{5.4.5}
\newcommand{\CrossrefCofibcatdefnwregularcleavageobj}{5.4.6}
\newcommand{\CrossrefCofibcatlemadmitframing}{5.4.7}
\newcommand{\CrossrefCofibcatthmapproxthm}{5.5.1}
\newcommand{\CrossrefCofibcateqnapproxarehtpyequiv}{5.1}
\newcommand{\CrossrefCofibcateqnapproxarehtpyequivXXY}{5.2}
\newcommand{\CrossrefCofibcateqnapproxarehtpyequivXXXY}{5.3}
\newcommand{\CrossrefCofibcatcorequivleftapprox}{5.5.3}
\newcommand{\CrossrefCofibcatcorotherleftapprox}{5.5.4}
\newcommand{\CrossrefCofibcatsectotalleftrightderived}{5.6}
\newcommand{\CrossrefCofibcatdefndeftotalleftkanextensions}{5.6.1}
\newcommand{\CrossrefCofibcatthmgeneralexistenceleftderived}{5.7.1}
\newcommand{\CrossrefCofibcateqnleftcleavage}{5.4}
\newcommand{\CrossrefCofibcateqnterminalproperty}{5.5}
\newcommand{\CrossrefCofibcateqnterminalpropertyXXXY}{5.6}
\newcommand{\CrossrefCofibcatcorgeneralexistenceleftderived}{5.7.2}
\newcommand{\CrossrefCofibcatthmgeneralexistencetotalderivedadjoint}{5.8.1}
\newcommand{\CrossrefCofibcatdefnabstractQuillenadjoint}{5.8.2}
\newcommand{\CrossrefCofibcateqnpartialadj}{5.7}
\newcommand{\CrossrefCofibcateqnpartialadjXXXY}{5.8}
\newcommand{\CrossrefCofibcateqnpartialadjXXXXY}{5.9}
\newcommand{\CrossrefCofibcatthmgeneralexistencetotalderivedadjointXXXY}{5.8.3}
\newcommand{\CrossrefCofibcatdefnabstractQuillenadjointXXXY}{5.8.4}
\newcommand{\CrossrefCofibcateqngeneraladjXXYXXY}{5.10}
\newcommand{\CrossrefCofibcateqngeneraladjXXYXXXY}{5.11}
\newcommand{\CrossrefCofibcatchaphomotcat}{6}
\newcommand{\CrossrefCofibcatseccofapproximations}{6.1}
\newcommand{\CrossrefCofibcatdefncofapproximation}{6.1.1}
\newcommand{\CrossrefCofibcatdefnfibapproximation}{6.1.2}
\newcommand{\CrossrefCofibcatlemweakequivcancelation}{6.1.3}
\newcommand{\CrossrefCofibcatlemcleavagechoice}{6.1.4}
\newcommand{\CrossrefCofibcatthmcofapproxareleftapprox}{6.1.5}
\newcommand{\CrossrefCofibcatthmcatcofobjequiv}{6.1.6}
\newcommand{\CrossrefCofibcatthmhomotopycatequiv}{6.1.7}
\newcommand{\CrossrefCofibcatremintermediatecofcat}{6.1.8}
\newcommand{\CrossrefCofibcatremintermediatecofcatXXXY}{6.1.9}
\newcommand{\CrossrefCofibcatsecleftrightderivedcofcat}{6.2}
\newcommand{\CrossrefCofibcatthmexistenceleftderived}{6.2.1}
\newcommand{\CrossrefCofibcatthmexistenceleftderivedapprox}{6.2.2}
\newcommand{\CrossrefCofibcatthmexistenceleftderivedequiv}{6.2.3}
\newcommand{\CrossrefCofibcatdefnquillenadjoint}{6.2.4}
\newcommand{\CrossrefCofibcatthmquillenadjoint}{6.2.5}
\newcommand{\CrossrefCofibcatchaphomotopicmaps}{6.3}
\newcommand{\CrossrefCofibcateqnlefthomotopy}{6.1}
\newcommand{\CrossrefCofibcateqnrighthomotopy}{6.2}
\newcommand{\CrossrefCofibcatthmhomotmaps}{6.3.1}
\newcommand{\CrossrefCofibcatlemchoosecyl}{6.3.2}
\newcommand{\CrossrefCofibcatthmhomotopyequivrel}{6.3.3}
\newcommand{\CrossrefCofibcatchaphomotopycalcoffractions}{6.4}
\newcommand{\CrossrefCofibcatthmgabrielzisman}{6.4.1}
\newcommand{\CrossrefCofibcateqngabrielzismanhypothesisXXY}{6.3}
\newcommand{\CrossrefCofibcateqndescrhomotopyXXY}{6.4}
\newcommand{\CrossrefCofibcatthmgabrielzismanXXXY}{6.4.2}
\newcommand{\CrossrefCofibcateqngabrielzismanhypothesisXXXY}{6.5}
\newcommand{\CrossrefCofibcateqndescrhomotopyXXXY}{6.6}
\newcommand{\CrossrefCofibcatthmhomotopycalcoffrations}{6.4.3}
\newcommand{\CrossrefCofibcatthmdescrhomot}{6.4.4}
\newcommand{\CrossrefCofibcatthmdescrhomotcof}{6.4.5}
\newcommand{\CrossrefCofibcatprophomotopyconsistence}{6.4.6}
\newcommand{\CrossrefCofibcatchaphomcalsappl}{7}
\newcommand{\CrossrefCofibcatchapprodcofcat}{7.1}
\newcommand{\CrossrefCofibcatthmprodhomotopycat}{7.1.1}
\newcommand{\CrossrefCofibcatsecsaturation}{7.2}
\newcommand{\CrossrefCofibcatlemcofcatequivinhomotcat}{7.2.1}
\newcommand{\CrossrefCofibcatlemcofcatissat}{7.2.2}
\newcommand{\CrossrefCofibcatthmcofcatissat}{7.2.3}
\newcommand{\CrossrefCofibcatthmquillensaturatedweq}{7.2.4}
\newcommand{\CrossrefCofibcatdefnXXXYoutofXXXXXXXY}{7.2.5}
\newcommand{\CrossrefCofibcatdefnweaksaturation}{7.2.6}
\newcommand{\CrossrefCofibcatthmcofcatissatXXXY}{7.2.7}
\newcommand{\CrossrefCofibcatthmcofcatsaturation}{7.2.8}
\newcommand{\CrossrefCofibcatproprightliftpropisweakequiv}{7.2.9}
\newcommand{\CrossrefCofibcatlemcofcatequivinhomotcatproper}{7.2.10}
\newcommand{\CrossrefCofibcatpropleftpropermapsaturated}{7.2.11}
\newcommand{\CrossrefCofibcatthmcofcatsaturationproper}{7.2.12}
\newcommand{\CrossrefCofibcatsecpim}{7.3}
\newcommand{\CrossrefCofibcatdefnfibrmodel}{7.3.1}
\newcommand{\CrossrefCofibcatpropsmallhomotopycat}{7.3.2}
\newcommand{\CrossrefCofibcatpropsmallhomotopycatXXXY}{7.3.3}
\newcommand{\CrossrefCofibcatpropsmallhomotopycatbaues}{7.3.4}
\newcommand{\CrossrefCofibcatpropsmallhomotopycatbauesXXY}{1}
\newcommand{\CrossrefCofibcatcorsmallhomotopycat}{7.3.5}
\newcommand{\CrossrefCofibcatlemdescrhomotopyquillen}{7.4.1}
\newcommand{\CrossrefCofibcatthmcharactproperness}{7.5.1}
\newcommand{\CrossrefCofibcateqnthmcharactproperness}{7.1}
\newcommand{\CrossrefCofibcatthmcharactpropernessquillen}{7.5.2}
\newcommand{\CrossrefCofibcatchapconstrcat}{8}
\newcommand{\CrossrefCofibcatsecbasicdefnotations}{8.1}
\newcommand{\CrossrefCofibcatsecinitterminalcat}{8.1.1}
\newcommand{\CrossrefCofibcatseccatinverseimage}{8.1.2}
\newcommand{\CrossrefCofibcatseccatdiag}{8.1.3}
\newcommand{\CrossrefCofibcatsecrelativelimcolim}{8.2}
\newcommand{\CrossrefCofibcatlemcomputerelcolim}{8.2.1}
\newcommand{\CrossrefCofibcatlemcolimcomposition}{8.2.2}
\newcommand{\CrossrefCofibcatsecsimplindex}{8.3}
\newcommand{\CrossrefCofibcatseccatnerve}{8.4}
\newcommand{\CrossrefCofibcatseccoffunctorsXXY}{8.5}
\newcommand{\CrossrefCofibcatdefncoffunct}{8.5.1}
\newcommand{\CrossrefCofibcatlemadjfunctcofinalfunct}{8.5.2}
\newcommand{\CrossrefCofibcatpropcofinallimitconv}{8.5.3}
\newcommand{\CrossrefCofibcatpropcofinallimit}{8.5.4}
\newcommand{\CrossrefCofibcateqncofinalcolimitiso}{8.1}
\newcommand{\CrossrefCofibcatsecgrothendieckconstruction}{8.6}
\newcommand{\CrossrefCofibcatpropgrothendieckconstructionadjoint}{8.6.1}
\newcommand{\CrossrefCofibcatpropgrothendieckconstrcolims}{8.6.2}
\newcommand{\CrossrefCofibcatcorgrothendieckconstrcolims}{8.6.3}
\newcommand{\CrossrefCofibcatremgrothendieckconstrcolims}{8.6.4}
\newcommand{\CrossrefCofibcatchaplimcolimcofinal}{9}
\newcommand{\CrossrefCofibcatseccatdirinv}{9.1}
\newcommand{\CrossrefCofibcatdefdirectinvcat}{9.1.1}
\newcommand{\CrossrefCofibcatdeflatchingmatchingcat}{9.1.2}
\newcommand{\CrossrefCofibcateqnlatchlatch}{9.1}
\newcommand{\CrossrefCofibcateqnmatchmatch}{9.2}
\newcommand{\CrossrefCofibcatdeflatchingmatchingobject}{9.1.3}
\newcommand{\CrossrefCofibcatsecreedycofstruct}{9.2}
\newcommand{\CrossrefCofibcatdefpointwisecof}{9.2.1}
\newcommand{\CrossrefCofibcatdefreedycof}{9.2.2}
\newcommand{\CrossrefCofibcatpropreedycofformcat}{9.2.3}
\newcommand{\CrossrefCofibcatthmreedycofibstruct}{9.2.4}
\newcommand{\CrossrefCofibcatseccolimdirectabsolute}{9.3}
\newcommand{\CrossrefCofibcatlemcolimpushout}{9.3.1}
\newcommand{\CrossrefCofibcatlemcolimpushoutset}{9.3.2}
\newcommand{\CrossrefCofibcatlemcompospushout}{9.3.3}
\newcommand{\CrossrefCofibcatlemcompospushoutXXXY}{9.3.4}
\newcommand{\CrossrefCofibcatthmcolimdirect}{9.3.5}
\newcommand{\CrossrefCofibcateqncolimreedycofXXXXY}{9.3}
\newcommand{\CrossrefCofibcateqncolimreedycofXXXXXXY}{9.4}
\newcommand{\CrossrefCofibcateqncolimreedycofXXXXXXXY}{9.5}
\newcommand{\CrossrefCofibcatcorcolimdirectcorollary}{9.3.6}
\newcommand{\CrossrefCofibcatdefnrestricteddiagrams}{9.3.7}
\newcommand{\CrossrefCofibcatthmreedycofibstructXXXY}{9.3.8}
\newcommand{\CrossrefCofibcatseccolimdirectrelative}{9.4}
\newcommand{\CrossrefCofibcatthmcolimdirectemb}{9.4.1}
\newcommand{\CrossrefCofibcateqncolimreedycofXXXXYbis}{9.6}
\newcommand{\CrossrefCofibcatthmcolimfromdirectcat}{9.4.2}
\newcommand{\CrossrefCofibcatthmcolimpairdirectcat}{9.4.3}
\newcommand{\CrossrefCofibcatseccolimarbitrarycat}{9.5}
\newcommand{\CrossrefCofibcatlemdeltaprimeovercat}{9.5.1}
\newcommand{\CrossrefCofibcatlemdeltaprimelcofinal}{9.5.2}
\newcommand{\CrossrefCofibcatlemrestrictedreedycofibrant}{9.5.3}
\newcommand{\CrossrefCofibcateqnclaimindstep}{9.7}
\newcommand{\CrossrefCofibcatproprestrictedproperty}{9.5.4}
\newcommand{\CrossrefCofibcatthmgeneralpointwisecofstructure}{9.5.5}
\newcommand{\CrossrefCofibcatthmgeneralpointwisecofibstructXXXY}{9.5.6}
\newcommand{\CrossrefCofibcatpropgeneralpointwisecofstructureapprox}{9.5.7}
\newcommand{\CrossrefCofibcatthmpointwisecofstructureequivalence}{9.5.8}
\newcommand{\CrossrefCofibcatsechocolimcolimdirect}{9.6}
\newcommand{\CrossrefCofibcatdefnhomotopycolim}{9.6.1}
\newcommand{\CrossrefCofibcatlemhomotcatcolim}{9.6.2}
\newcommand{\CrossrefCofibcatthmgenholim}{9.6.3}
\newcommand{\CrossrefCofibcatcorcomposhomotcolimits}{9.6.4}
\newcommand{\CrossrefCofibcateqnXXXYcatsquareXXXXXY}{9.8}
\newcommand{\CrossrefCofibcateqnstdoverXXXYcat}{9.9}
\newcommand{\CrossrefCofibcateqnhomotopycolimbasechange}{9.10}
\newcommand{\CrossrefCofibcateqnstdunderXXXYcat}{9.11}
\newcommand{\CrossrefCofibcateqnhomotopylimbasechange}{9.12}
\newcommand{\CrossrefCofibcatthmcomputerelhocolim}{9.6.5}
\newcommand{\CrossrefCofibcatthmopenembeddingdiagrams}{9.6.6}
\newcommand{\CrossrefCofibcatlemleftadjointoflcolimXXY}{9.6.7}
\newcommand{\CrossrefCofibcatlemleftadjointoflcolimXXXY}{9.6.8}
\newcommand{\CrossrefCofibcatthmleftadjointoflcolim}{9.6.9}
\newcommand{\CrossrefCofibcatsecconservationproperty}{9.7}
\newcommand{\CrossrefCofibcatthmhomotcatconservative}{9.7.1}
\newcommand{\CrossrefCofibcateqndgm}{9.13}
\newcommand{\CrossrefCofibcatcorhomotcatconservative}{9.7.2}
\newcommand{\CrossrefCofibcatsecrealizingdiagrams}{9.8}
\newcommand{\CrossrefCofibcatlemdescrfinitefreecat}{9.8.1}
\newcommand{\CrossrefCofibcatlemcofcatsumsofdiagrams}{9.8.2}
\newcommand{\CrossrefCofibcatlemcofcathomotopysum}{9.8.3}
\newcommand{\CrossrefCofibcatlemsufficientfinitefull}{9.8.4}
\newcommand{\CrossrefCofibcatthmfreedirectdiagramrealization}{9.8.5}
\newcommand{\CrossrefCofibcatthmexistenceweakcolimits}{9.8.6}
\newcommand{\CrossrefCofibcatchapderivators}{10}
\newcommand{\CrossrefCofibcatsecpreder}{10.1}
\newcommand{\CrossrefCofibcatdefnhellerpreder}{10.1.1}
\newcommand{\CrossrefCofibcatsecder}{10.2}
\newcommand{\CrossrefCofibcateqnXXXYcatsquareder}{10.1}
\newcommand{\CrossrefCofibcateqnXXXYcatsquaredermap}{10.2}
\newcommand{\CrossrefCofibcateqnXXXYcatsquaredermapop}{10.3}
\newcommand{\CrossrefCofibcateqnstdoverXXXYcatbasechangedgm}{10.4}
\newcommand{\CrossrefCofibcateqnstdoverXXXYcatbasechange}{10.5}
\newcommand{\CrossrefCofibcateqnstdoverXXXYcatcobasechangedgm}{10.6}
\newcommand{\CrossrefCofibcateqnstdunderXXXYcatcobasechange}{10.7}
\newcommand{\CrossrefCofibcatdefnhellerderivator}{10.2.1}
\newcommand{\CrossrefCofibcatdefngrothderivator}{10.2.2}
\newcommand{\CrossrefCofibcatdefnhellerstrongderivator}{10.2.3}
\newcommand{\CrossrefCofibcatthmhellerderishtpytheory}{10.2.4}
\newcommand{\CrossrefCofibcatsecderivability}{10.3}
\newcommand{\CrossrefCofibcatdefnderivablecat}{10.3.1}
\newcommand{\CrossrefCofibcatthmcofcatderivator}{10.3.2}
\newcommand{\CrossrefCofibcatthmmodelcatderivator}{10.3.3}
\newcommand{\CrossrefCofibcatsecoddsandends}{10.4}
\newcommand{\CrossrefCofibcatthmcofcatderivatorXXXY}{10.4.1}


==> definitions.tex <==
%\documentclass[12pt]{amsart}
\usepackage{amscd}
\usepackage{amsmath,amsthm}     % Handy math stuff, theorem environments.
\usepackage{amssymb}
\usepackage{euscript}           % Nice script font.
\usepackage[all,2cell,ps]{xy} \UseAllTwocells \SilentMatrices
%\usepackage{makeidx}
\CompileMatrices		% speeds up XY-pic diagram compilation
\UseComputerModernTips		% use Knuth's computer modern fonts

% Comment out before distribution - 
%\usepackage{showkeys}  % Enables the labels in text.
%\usepackage{hyperref}  % Hyperlinks

% Comment in for smaller page margin
%\addtolength{\oddsidemargin}{-1cm}
%\addtolength{\evensidemargin}{-1cm}
%\addtolength{\headheight}{0pt}
%\addtolength{\headsep}{0cm}
%\addtolength{\textheight}{0cm}
%\addtolength{\textwidth}{2cm}
%\addtolength{\footskip}{0cm}

%\parskip1ex 


%%% This part of the file (after the \documentclass command,
%%% but before the \begin{document}) is called the ``preamble''.
%%% This is a good place to  put our macro definitions.

\newcommand{\tensor}{\otimes}
\newcommand{\homotopic}{\simeq}
\newcommand{\homeq}{\cong}
\newcommand{\iso}{\approx}

\DeclareMathOperator{\ho}{Ho}

\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}

\newcommand{\M}{\mathcal{M}}
\newcommand{\W}{\mathcal{W}}

\newcommand{\itilde}{\tilde{\imath}}
\newcommand{\jtilde}{\tilde{\jmath}}
\newcommand{\ihat}{\hat{\imath}}
\newcommand{\jhat}{\hat{\jmath}}
\newcommand{\comment}[1]{}

\newcommand{\cat}[1]{\EuScript {#1}}
\newcommand{\axiom}[1]{\textbf {#1}}

% arrows
\newcommand{\lra}{\longrightarrow}
\newcommand{\lla}{\longleftarrow}
\newcommand{\ra}{\rightarrow}
\newcommand{\la}{\leftarrow}
\newcommand{\llra}{\longleftrightarrow}
\newcommand{\dbra}{\rightrightarrows}           % double arrow for equalizer diagrams
\newcommand{\Ra}{\Rightarrow}
\newcommand{\La}{\Leftarrow}

% dots
%\newcommand{\tdot}{^{^\centerdot}} 	% upper dot
\newcommand{\tdot}{^{^{_{_\bullet}}}} 	% upper dot
\newcommand{\tdotdot}{^{^{_{_{\bullet\bullet}}}}}
%\newcommand{\sdot}{_\centerdot}			% lower dot
\newcommand{\sdot}{_{_{^{^\bullet}}}} 	% upper dot
\newcommand{\sdotdot}{_{_{^{^{\bullet\bullet}}}}} 	% upper dot

%math symbols
\newcommand{\comp}{\circ}

%special faces & letters
\newcommand{\eps}{\epsilon}
\newcommand{\epso}{\overline \epsilon}
\newcommand{\nuo}{\overline \nu}
\newcommand{\Deltao}{\overline \Delta} 
\newcommand{\Mo}{\overline M} 

%completion
\newcommand{\compl}[1]{{#1}\,{\hat{}}_{\!\!\!R}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newdir{ >}{{}*!/-5pt/\dir{>}}                  % Make better tailed arrows.
\newdir{ |}{{}*!/-5pt/\dir{|}}                  % Make better mapsto arrows.

% Some theorem-like environments, all numbered together starting at 1
% in each section.

\newcommand{\mdfn}[1]{\dfn{\mathversion{bold}#1}} % Even make math symbols bold

% Topologists smash /\ and wedge \/.
\newcommand{\Smash}             {\wedge}
\newcommand{\bigSmash}          {\bigwedge}
\newcommand{\hfsm}              {\rtimes}
\newcommand{\eqhsma}[1]{\underset{\Sigma_{#1}}  %`equivariant half-smash'---
                                 {\rtimes}}     %\eqhsma{n} produces the symbol
                                                %`half-smash over sigma_n'
\newcommand{\eqtens}[1]{\underset{\Sigma_{#1}}  %`equivariant tensor' 
                                 {\otimes}}
% For fibred products. Modify this to something fancier if desired.
% "arg1 multiplied over arg2 with arg3"
\newcommand{\fibpr}[3]{{#1}\times_{#2}{#3}}

% produces a times symbol with a subscript directly beneath it, rather
% than beneath and to the right.
\newcommand{\timessub}[1]{\underset{#1}{\times}}

% same, but with otimes
\newcommand{\otimessub}[1]{\underset{#1}{\otimes}}

\newcommand{\und}{\underline}
\newcommand{\norm}[1]{\mid #1 \mid}
\newcommand{\Sum} {\sqcup}
\newcommand{\Wedge} {\vee}
\DeclareRobustCommand{\bigWedge}{\bigvee}
\DeclareMathOperator*{\invlim}{\varprojlim}
\DeclareMathOperator*{\dirlim}{\varinjlim}
\DeclareMathOperator*{\colim}{colim\,}
\DeclareMathOperator*{\wcolim}{wcolim\,}
\DeclareMathOperator*{\wlim}{wlim\,}
\DeclareMathOperator*{\initial}{{\bf 0}}
\DeclareMathOperator*{\final}{{\bf 1}}
\DeclareMathOperator*{\terminal}{\final}
\DeclareMathOperator*{\initialcat}{\emptyset}
\DeclareMathOperator*{\finalcat}{{\it e}}
\DeclareMathOperator*{\terminalcat}{\finalcat}

\newcommand{\corollaryref}[1] {Cor. \ref{#1}}
\newcommand{\definitionref}[1] {Def. \ref{#1}}
\newcommand{\lemmaref}[1] {Lemma \ref{#1}}
\newcommand{\propositionref}[1] {Prop. \ref{#1}}
\newcommand{\theoremref}[1] {Thm. \ref{#1}}
\newcommand{\conjectureref}[1] {Conj. \ref{#1}}
\newcommand{\remarkref}[1] {Remark \ref{#1}}
\newcommand{\chapterref}[1] {Chap. \ref{#1}}
\newcommand{\sectionref}[1] {Section \ref{#1}}
\newcommand{\equationref}[1] {(\ref{#1})}


% The following causes equations to be numbered within sections
%\newcounter{theoremcounter}
%\numberwithin{theoremcounter}{subsection}
%\numberwithin{equation}{section}

%\theoremstyle{plain} %% This is the default, anyway
%\newtheorem{thm}[theoremcounter]{Theorem}
%\newtheorem{cor}[theoremcounter]{Corollary}
%\newtheorem{lem}[theoremcounter]{Lemma}
%\newtheorem{prop}[theoremcounter]{Proposition}
%\newtheorem{conjecture}[theoremcounter]{Conjecture}
%\theoremstyle{definition}
%\newtheorem{defn}[theoremcounter]{Definition}
%\theoremstyle{remark}
%\newtheorem{rem}[theoremcounter]{Remark}
%\newtheorem{ex}[theoremcounter]{Example}
%\newtheorem{notation}[theoremcounter]{Notation}
%\newtheorem{terminology}[theoremcounter]{Terminology}


==> theorem-environment.tex <==
\newcounter{theoremcounter}
%\numberwithin{theoremcounter}{section}
%\numberwithin{section}{chapter}
%\numberwithin{equation}{chapter}
\theoremstyle{plain} %% This is the default, anyway
\newtheorem{thm}[theoremcounter]{Theorem}
\newtheorem{cor}[theoremcounter]{Corollary}
\newtheorem{lem}[theoremcounter]{Lemma}
\newtheorem{prop}[theoremcounter]{Proposition}
\newtheorem{conjecture}[theoremcounter]{Conjecture}
\newtheorem{open-issue}[theoremcounter]{Open Issue}
\theoremstyle{definition}
\newtheorem{defn}[theoremcounter]{Definition}
\theoremstyle{remark}
\newtheorem{rem}[theoremcounter]{Remark}
\newtheorem{ex}[theoremcounter]{Example}
\newtheorem{notation}[theoremcounter]{Notation}
\newtheorem{terminology}[theoremcounter]{Terminology}

